iMTSP: Solving Min-Max Multiple Traveling Salesman Problem with Imperative Learning

This paper considers a Min-Max Multiple Traveling Salesman Problem (MTSP), where the goal is to find a set of tours, one for each agent, to collectively visit all the cities while minimizing the length of the longest tour. Though MTSP has been widely studied, obtaining near-optimal solutions for large-scale problems is still challenging due to its NP-hardness. Recent efforts in data-driven methods face challenges of the need for hard-to-obtain supervision and issues with high variance in gradient estimations, leading to slow convergence and highly suboptimal solutions. We address these issues by reformulating MTSP as a bilevel optimization problem, using the concept of imperative learning (IL). This involves introducing an allocation network that decomposes the MTSP into multiple single-agent traveling salesman problems (TSPs). The longest tour from these TSP solutions is then used to self-supervise the allocation network, resulting in a new self-supervised, bilevel, end-to-end learning framework, which we refer to as imperative MTSP (iMTSP). Additionally, to tackle the high-variance gradient issues during the optimization, we introduce a control variate-based gradient estimation algorithm. Our experiments showed that these innovative designs enable our gradient estimator to converge 20% faster than the advanced reinforcement learning baseline and find up to 80% shorter tour length compared with Google OR-Tools MTSP solver, especially in large-scale problems (e.g. 1000 cities and 15 agents).

==> backup.tex <==


% Because of its NP-hard nature, MTSP is very challenging.
% It is known for its issue of combinatorial explosion, e.g., an MTSP with $100$ cities and $10$ agents has $\frac{100!99!}{10!\times89!} \approx10^{20000}$ possible solutions. As a comparison, the observable universe contains ``merely'' about $10^{78}$ to $10^{82}$ atoms \cite{gaztanaga2023mass}.
% Additionally, unlike the classic traveling salesman problem (TSP), which focuses on minimizing the total distance traveled by a single agent, MTSP involves minimizing the maximum distance traveled by any agent. This adds additional complexity because it requires balancing multiple routes to ensure that no single route is excessively long compared to others.
% Comparing with the well-known sophisticated game Go, whose number of possible situations is $361!$ ($361$ feasible positions), the number of an MTSP with $361$ cities and $10$ agents has $\frac{(360!)^2}{10!\times350!}$ possible solutions, which is approximately $2\times10^{15}$ times more complex.
% Despite its complexity, MTSP is a concise mathematical abstraction of many important topics such as unmanned aerial vehicles~\cite{sundar2013algorithms, ma2019coordinated}, automated agriculture~\cite{carpio2021mp}, warehouse logistics~\cite{wurman2008coordinating,10109784}. % In its basic version, multiple agents need to visit multiply nodes, where each node needs to be visit one and only one time by one of the agents. The objective could be the length of the longest route or the length of the total traveling distance. 
% As naive as the problem sounds like, 
% and is computational difficult in large scales. Making the problem even harder, various constrains could be attached to the basic version. 
% This problem can be extended by considering more complex constraints, such as cities' visiting time window~\cite{wang2020ant}, and agent's maximum traveling distance.

% Extensive studies have been conducted from various perspectives. In pursuit of optimal solutions, some researchers proposed analytical solutions for MTSP or its variations.~\cite{ham2018integrated,ren2021ms}. Such approaches fall short in dealing with large scale problems but provide a guide line for further studies. Heuristic algorithm 

%Additionally, further complexity arises in MTSP compared to the classic Traveling Salesman Problem (TSP), which aims to minimize the total distance traveled by a single agent.
% The Min-Max MTSP continues to present significant challenges, and
